Semi-Self Representation Learning for Crowdsourced WiFi Trajectories

WiFi fingerprint-based localization has been studied intensively. Point-based solutions rely on position annotations of WiFi fingerprints. Trajectory-based solutions, however, require end-position annotations of WiFi trajectories, where a WiFi trajectory is a multivariate time series of signal features. A trajectory dataset is much larger than a pointwise dataset as the number of potential trajectories in a field may grow exponentially with respect to the size of the field. This work presents a semi-self representation learning solution, where a large dataset $C$ of crowdsourced unlabeled WiFi trajectories can be automatically labeled by a much smaller dataset $\tilde C$ of labeled WiFi trajectories. The size of $\tilde C$ only needs to be proportional to the size of the physical field, while the unlabeled $C$ could be much larger. This is made possible through a novel ``cut-and-flip'' augmentation scheme based on the meet-in-the-middle paradigm. A two-stage learning consisting of trajectory embedding followed by endpoint embedding is proposed for the unlabeled $C$. Then the learned representations are labeled by $\tilde C$ and connected to a neural-based localization network. The result, while delivering promising accuracy, significantly relieves the burden of human annotations for trajectory-based localization.

==> arxiv/macros.tex <==
% Lai-macros.tex

\newcommand\PP{\bigskip\noindent}

\newcommand\st{\textstyle \ast}
\newcommand{\dott}{\thinspace\ldotp\ldotp}
\newcommand\defeq{\stackrel{\rm def}{=}}
%\newcommand\proof{\noindent {\bf Proof}. }
%\newcommand\qed{\hfill $\Box$ \smallskip}
%\newcommand\qed{\hspace*{\fill} $\Box$ \smallskip}
\newcommand{\blist}{\begin{list}\setlength{\topsep 0pt \parsep 0pt}}
\newcommand{\elist}{\end{list}}
\newtheorem{thm}{Theorem}
\newcommand{\bthm}{\begin{thm}\begin{textit}}
\newcommand{\ethm}{\end{textit}\end{thm}}
\newtheorem{dfn}{Definition}
\newcommand{\bdfn}{\begin{dfn}\begin{textit}}
\newcommand{\edfn}{\end{textit}\end{dfn}}
\newtheorem{obn}{Observation}
\newcommand{\bobn}{\begin{obn}\begin{textit}}
\newcommand{\eobn}{\end{textit}\end{obn}}
\newtheorem{prop}{Proposition}
\newtheorem{lema}{Lemma}
\newcommand{\bdla}{\begin{lema}\begin{textit}}
\newcommand{\edla}{\end{textit}\end{lema}}
\newtheorem{pro}{Property}
\newcommand{\bpro}{\begin{pro}\begin{textit}}
\newcommand{\epro}{\end{textit}\end{pro}}
\newtheorem{cor}{Corollary}
\newtheorem{conj}{Conjecture}
\newtheorem{ex}{Example}
%\newcommand{\mod}{\mbox{mod}}
%\newcommand{\mod}{\mathop{\mathrm{mod}}}
\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcounter{algnum1}
\newenvironment{rlist}
{\begin{list}{(\roman{algnum1})}
{\usecounter{algnum1}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

\newcounter{algnum2}
\newenvironment{alist}
{\begin{list}{(\alph{algnum2})}
{\usecounter{algnum2}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\leftmargin 0.3in}
 \setlength{\labelsep 5pt}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

\newcounter{algnum3}
\newenvironment{Alist}
{\begin{list}{A\alph{algnum3}.}
{\usecounter{algnum3}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\leftmargin 0.3in}
 \setlength{\labelsep 5pt}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

%\setlength{\textwidth}{6.1 in}
%\setlength{\textheight}{8.5in}
%\hoffset=-0.45in % 10 pts
%\voffset=-.5in
%\hoffset=-0.55in  % 11 pts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tseng-macros.tex

\newcommand\myqed{\hspace*{\fill} \smallskip $\rule{2mm}{2mm}$}
\newcommand\cspbox{[\hspace{-1pt}]}
\newcommand\eqdef{\stackrel{def}{=}}
\newcommand\algoskip{\parskip=0pt \parsep=0pt \itemsep=0pt}

\newcommand\lc{\lceil}
\newcommand\rc{\rceil}
\newcommand\lf{\lfloor}
\newcommand\rf{\rfloor}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\ul{\underline}
\newcommand\ol{\overline}
\newcommand\bit{\begin{itemize}}
\newcommand\eit{\end{itemize}}
\newcommand\itcompress{\parskip=0pt \parsep=0pt \itemsep=0pt}

\newcommand{\Dfn}[1]{Definition~\ref{#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{#1}) and (\ref{#2})}
\newcommand{\Ex}[1]{Example~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Figs}[2]{Figs.~\ref{#1} and \ref{#2}}
\newcommand{\Lema}[1]{Lemma~\ref{#1}}
\newcommand{\Pro}[1]{pro~\ref{#1}}
\newcommand{\Thm}[1]{Theorem~\ref{#1}}
\newcommand{\Cor}[1]{Corollary~\ref{#1}}
\newcommand{\Prop}[1]{Proposition~\ref{#1}}
\newcommand{\Chap}[1]{Chapter~\ref{#1}}
\newcommand{\Sec}[1]{Section~\ref{#1}}
\newcommand{\Tab}[1]{Table~\ref{#1}}
\newcommand{\Tabs}[2]{Tables~\ref{#1} and \ref{#2}}
\newcommand{\App}[1]{Appendix~\ref{#1}}

\newenvironment{dlist}
{\begin{list}{xxxxxx}{}
}
{\end{list}}


%\mathchardef\bullet=220F               % if no bullets shows, try this

\newcommand{\normalparskip}{\parskip 10pt}
\newcommand{\tideparskip}{\parskip 6pt}
\newcommand{\doublespace}{\baselineskip=22pt}
\newcommand{\tidespace}{\baselineskip=12pt}
\newcommand{\singlespace}{\baselineskip=16pt}
\newcommand{\widespace}{\baselineskip=30pt}

\newenvironment{llist}{\begin{list}{}{\setlength
        \labelwidth{.6in}\setlength\leftmargin{\labelwidth}\addtolength
        \leftmargin{\labelsep}\itemsep 5pt plus 2pt minus 2pt
        \parsep 5pt plus 2pt minus 2pt
        \def\ITEM##1{\item[{##1}]}
        \def\makelabel##1{##1\hfill}}}{\end{list}}
\newenvironment{idescription}{\begin{list}{}{\listparindent=0.25in}
        \def\Item##1{\item[{\bf ##1}]}
        }{\end{list}}

\newcommand{\ouraddress}{
        Department of Computer and Information Science\\
        The Ohio State University\\
        2036 Neil Avenue\\
        Columbus, OH 43210-1277\\
        Tel:(614)292-6552\\
        Fax:(614)292-9201\\
        E-mail: liu@cis.ohio-state.edu
}

% Define double brackets
%
\newcommand{\ldb}{[\hspace{-2pt}[}      % left double bracket
\newcommand{\rdb}{]\hspace{-2pt}]}      % right double bracket
\newcommand{\bldb}{{\bf\ldb}}           % bold face left double bracket
\newcommand{\brdb}{{\bf\rdb}}           % bold face right double bracket
\newcommand{\db}[1]{\ldb{#1}\rdb}       % item quoted by double brckets
\newcommand{\bdb}[1]{\bldb{#1}\brdb}    % item quoted by bold face
                                        % double breckets

% Usage: \balgo ... \ealgo
\newcommand{\balgo}{
   \begin{description}
   \parskip=0pt
   \topsep=0pt
}
\newcommand{\ealgo}{
   \end{description}
}

%\newcommand{\algorithm}[4]{
%        \begin{scriptsize}
%        \begin{tabbing}
%                {\bf Procedure} #1 \\
%        XXX\={\bf output:}X\= \+\kill
%        {\bf input:}\>\+ #2\-\\
%        {\bf output:}\>\+ #3\-\\[0.1in]
%        XXX\=XXX\=XXX\=XXX\=XXX\=XXX\=\kill
%        #4 \-\\
%        {\bf end};
%        \end{tabbing}
%        \end{scriptsize}
%}
\newcommand{\while}[2]{
        {\bf while} (#1) {\bf do}\+\\
        #2\-\\
        {\bf end-while}
}
\newcommand{\for}[2]{
        {\bf for} (#1) {\bf do}\+\\
        #2\-\\
        {\bf end-for}
}
\newcommand{\ifthen}[2]{
        {\bf if} (#1) {\bf then}\+\\
        #2\-\\
        {\bf end-if}
}
%\newcommand{\ifthenelse}[3]{
%        {\bf if} (#1) {\bf then}\+\\
%        #2\-\\
%        {\bf else}\+\\
%        #3\-\\
%        {\bf end-if}
%}
\newcommand{\rptuntil}[2]{
        {\bf repeat}\+\\
        #1\-\\
        {\bf until} (#2)
}
\newcommand{\return}[1]{{\bf return} #1}
\newcommand{\ass}{$\leftarrow$}

%
% Define algorithm commands
%
% Usage: the algorithm with only input, but no output,
%       \inalgorithm{<name>}{<input parameters>}{<the algorithms>}
%       \while{<condition>}{<while loop body>}
%       \for{<condition>}{<for loop body>}
%       \ifthen{<condition>}{<then part>}
%       \ifthenelse{<condition>}{<then part>}{<else part>}
%       \rptuntil{<loop body>}{<condition>}
%
\newcommand{\inalgorithm}[3]{
        \begin{small}
        \begin{tabbing}
                {\bf Procedure} #1 \\
        {\bf input:}X\=  \kill
        {\bf input:}\>\+ #2\-\\
        {\bf begin} \\
        XXX\=XXX\=XXX\=XXX\=XXX\=XXX\=\kill
        #3 \\
        {\bf end}.
        \end{tabbing}
        \end{small}
}

